Towards a Mechanistic Understanding of Large Reasoning Models: A Survey of Training, Inference, and Failures

Reinforcement learning (RL) has catalyzed the emergence of Large Reasoning Models (LRMs) that have pushed reasoning capabilities to new heights. While their performance has garnered significant excitement, exploring the internal mechanisms driving these behaviors has become an equally critical research frontier. This paper provides a comprehensive survey of the mechanistic understanding of LRMs, organizing recent findings into three core dimensions: 1) training dynamics, 2) reasoning mechanisms, and 3) unintended behaviors. By synthesizing these insights, we aim to bridge the gap between black-box performance and mechanistic transparency. Finally, we discuss under-explored challenges to outline a roadmap for future mechanistic studies, including the need for applied interpretability, improved methodologies, and a unified theoretical framework.

==> paper/long_version_unintended_behaviors.tex <==
\section{Unintended Behaviors: Phenomena and Mechanisms}
\label{sec:special_behavior}
Beyond the enhancement of reasoning capabilities, RL induces a spectrum of other significant, and often unintended, behavioral effects. A comprehensive understanding of these phenomena is crucial for a holistic assessment of reasoning models. Key among these effects are the intention for \textbf{hallucination} (\S\ref{ssec:hallucination}), where models generate plausible but factually incorrect content; \textbf{CoT unfaithfulness} (\S\ref{ssec:faithfulness}), where the model's internal computation and CoT outputs diverge; and \textbf{overthinking} (\S\ref{ssec:overthink}), where models tend to generate unnecessarily long and redundant reasoning chains, resulting in computational inefficiency and potential performance degradation.

\subsection{Hallucination}
\label{ssec:hallucination}
The emergence of complex, multi-step reasoning chains in Large Reasoning Models (LRMs) has introduced new vulnerabilities to factual errors and hallucinations. These errors are often more insidious as they can be camouflaged within structured intermediate steps.

\paragraph{Do reasoning models hallucinate more?}
% Are Reasoning Models More Prone to Hallucination?
Recent evidence suggests that reasoning-oriented training pipelines can substantially affect hallucination behavior. \citet{are_reasoning_models-zijun} show that complete post-training pipelines which combine SFT with RLVR can alleviate hallucination. In contrast, incomplete pipelines, such as pure RL without cold start SFT or distillation-only approaches, tend to introduce more nuanced hallucinations.
However, \citep{lireasoning} indicates that reasoning-focused RL fine-tuning often increases the prevalence of hallucinations, even when SFT is included. Furthermore,~\citet{zhao2025test} shows that test-time scaling provides no consistent mitigation: for knowledge-intensive tasks, using more computation during inference does not reliably improve factual accuracy and frequently amplifies hallucinations.

\researchfinding{
  Growing evidence suggests reasoning models hallucinate more. However, there are debates whether models with complete post-training pipelnes hallucinate more.
}

\paragraph{Behavior analysis of reasoning model hallucination}
% behavior analysis
% \citet{are_reasoning_models-zijun}: Flaw repetition and think-answer mismatch are two important causes of hallucination for RL-only and SFT-only LRMs. (1) Flaw repetition, where the LRM is trapped in a loop of repeated thoughts. Those reasoning thoughts could be different in language surface but are semantically similar. Even though the required knowledge is encoded in the model parameters, the LRM fails to retrieve it because it cannot end thinking before running out of the context length limit. (2) Think-Answer mismatch, where the answer given by the LRM does not semantically align with its CoT.

% \textcolor{blue}{[Auditing Meta-Cognitive]}: The RLLM fails to accurately assess its metacognitive confidence in claims derived from incorrect knowledge, leading to the mistaken reinforcement of uncertain claims through reflective reasoning.\textit{ Hallucination Origin}: Hallucinations emerge from incorrect knowledge when the model overconfidently generates claims that it has not properly internalized, leading to the propagation of errors
% throughout the reasoning process. \textit{Hallucination Propagation.} Reflection in long-CoT reasoning amplifies hallucinations by reinforcing erroneous claims, with the metacognitive confidence increasing for these flawed
% claims despite their inaccuracy.

Recent analyses reveal that hallucinations in LRMs often stem from characteristic behavioral failure modes that arise during multi-step reasoning. \citet{are_reasoning_models-zijun} identify \emph{flaw repetition}, where the model becomes trapped in loops of semantically similar thoughts despite superficial linguistic variation, and \emph{think–answer mismatch}, where the final prediction does not align with the model’s own chain of thought. These issues frequently occur in RL-only or SFT-only models, causing the reasoning process to drift away from grounded facts. Complementary evidence from~\citet{lu2025auditing} shows that LRMs suffer from \emph{meta-cognitive failures}, where they tend to over-confidently generate claims that are derived from incorrect, un-internalized knowledge. This error propagates and is amplified by reflection in long-CoT reasoning, reinforcing the erroneous claims.

% mechanism analysis
\paragraph{Mechanism analysis of reasoning model hallucination.}
% \citet{are_reasoning_models-zijun}: increased hallucination of LRMs is usually associated with the misalignment between model uncertainty and factual accuracy. the SFT+RL pipeline helps to improve the calibration of LRMs, while the calibration of LRMs is corrupted by the SFT-only and RL-only post-training pipelines.

% \textcolor{blue}{[Detection and Mitigation]}: propose reasoning score to characterize the depth of reasoning by measuring the divergence between the logits obtained from early layers through logitlens and that from the final layer; the mechanism pattern of hallucination: 1) early stage fluctuation in reasoning depth, 2) incorrect backtracking to flawed prior steps, including shallow pattern-matching steps and overthinking steps

At a mechanistic level, hallucination in LRMs is closely tied to \emph{misalignment between model uncertainty and factual accuracy}. \citet{are_reasoning_models-zijun} show that complete post-training pipelines combining SFT and RL help restore calibration, allowing uncertainty estimates to better track correctness, whereas SFT-only and RL-only pipelines degrade calibration and thereby increase hallucination rates. Besides, \citet{sun2025detection} proposes a reasoning-depth score, which is measured through divergence between early-layer logits (via logit lens~\citep{lens2020}) and final-layer predictions, to quantify the internal depth of reasoning. Their analysis reveals that hallucinations often follow a consistent internal pattern: 1) \emph{fluctuations in reasoning depth during early steps}, and 2) \emph{backtracking to flawed prior thoughts}, including shallow pattern-matching steps and overthinking steps.
 
\paragraph{How does RL affect hallucination?}
% \textcolor{blue}{[The Hallucination Tax]}: RFT makes models more reluctant to abstain from answering a question, even when the query is factually unanswerable. (which is also reported in \textcolor{blue}{[Test-Time Scaling]})

% \textcolor{blue}{[Reasoning Models Hallucinate More]}: First, optimizing solely for correct final answers leads to extremely high variance in the policy gradient when such answers are rare, yielding unstable training updates. Second, the need to discover rewarding outputs forces the policy to maintain a high level of entropy in its predictions, heightening the risk of hallucinations. Third, standard RL objectives admit spurious local optima whereby the model can converge to a confidently held wrong answer that yields zero reward. These three factors, i.e., high-variance gradient, entropy-induced randomness, and spurious local optima, together explain why a purely outcome-based RL approach can cause a reasoning model to hallucinate and struggle to learn faithful reasoning patterns

RL introduces its own systematic pressures that shape hallucination behavior in reasoning models. \citet{song2025hallucination} shows that RL reduces a model’s willingness to abstain, pushing it to generate answers even for factually unanswerable questions, which is also observed in~\citet{zhao2025test}. Regarding the process of RL training, \citet{lireasoning} explains that  optimizing only for final-answer correctness creates extremely \emph{high-variance gradients} when correct outputs are sparse, leading to unstable updates; at the same time, RL’s need for exploration forces the model to maintain \emph{high entropy in its predictions}, increasing the likelihood of hallucinations during reasoning. Furthermore, standard RL objectives can drive the policy toward \emph{spurious local optima} where the model confidently adopts incorrect but zero-reward answers. Together, the factors including high-variance gradient, entropy-induced randomness, and spurious local optima explain why RLVR can cause the reasoning models to hallucinate more.


\subsection{CoT faithfulness}
\label{ssec:faithfulness}
% One benefit of LRMs is that they naturally produces CoT along with the final answer, where we expect to monitor the long CoT to explain their inner mechanism of the model.
% By inspecting the long CoT, we can diagnose the model, such as identifying reward hacking or mis-behaviors.

As LRMs are natively equipped with extended intermediate CoT, it is expected that we can monitor their decision-making process by inspecting the long CoTs.
This is beneficial for multiple different purposes~\citep{monitorability-openai}.
For example, we can prevent malicious behaviors before the model generate the final outputs by inspecting their CoTs prior to answer generation~\citep{monitorability-openai, baker2025monitoring, chan2025can}.
However, whether the intermediate CoTs are faithful to the model's internal computation is still under debate~\citep{are_reasoning_models-zijun,dont_say_what_they_think-anthropic, chua2025deepseek, cot_in_the_wild_not_faithful, baker2025monitoring}.



\paragraph{Contextual Faithfulness of CoT in LRMs.}

% Although LRMs generate long CoTs before producing their final output, it remains unclear whether the generated CoTs are semantically consistent with the final output in the LRMs.
Several studies indicate that, despite generating the final output conditioned on the preceding CoT, the intermediate CoTs are not always semantically faithful to the final output.
For example, \citet{are_reasoning_models-zijun} identifies a phenomenon called \textit{Think-Answer Mismatch}, where the model's final answer contradicts its preceding CoT.
As we have mentioned in Section~\ref{ssec:hallucination}, this is considered as one of the cause of hallucination in LRMs, particularly in fact-seeking scenarios.

% \textcolor{blue}{[10]}:
To quantify contextual faithfulness of CoTs, \citet{chua2025deepseek} proposes to evaluate whether the LRMs can explicitly articulate input interventions that directly lead to changes in the final answer through their CoTs.
This is achieved by injecting hints implying an incorrect answer into the prompt.
For cases where the model initially answers correctly but changes its response after the intervention, they assess whether the CoT references the injected cues.
% \textcolor{blue}{[1]}:
Similarly, \citet{dont_say_what_they_think-anthropic} measure whether the LRMs verbalize the use of the provided hints in the prompts, when these cause the model to switch its final.
% \textcolor{blue}{[3]}:
\citet{cot_in_the_wild_not_faithful} studies another specific form of unfaithfulness, called \textit{``Implicit Post-Hoc Rationalization''} where models, due to their own implicit biases, generate logically contradictory ``Yes'' or ``No'' answers to opposite questions. They produce coherent-sounding rationalizations to justify these predetermined conclusions.

The studies collectively find that LRMs are more faithful to their intermediate CoTs than their non-reasoning backbones.
However, the faithfulness is still far from perfect. For example, \citet{dont_say_what_they_think-anthropic} finds that less than 20\% usage of the injected hints are verbalized in CoTs. 
% \textcolor{blue}{[5]}:
Additionally, \citet{wang2025thinking} shows that reasoning models can be induced to perform strategic deception---engaging in goal-driven, intentional misleading where the reasoning process contradicts outputs.
% 以上文章还有一些其他的小结论可以放，比如RL怎么影响faithfulness之类的，需要放进来吗？

\researchfinding{
  LRMs do not always generate semantically faithful CoTs that are consistent with their final output, but they are more faithful than non-reasoning models.
}


\paragraph{Mechanistic Understanding of CoT Faithfulness in LRMs.}
Beyond contextual faithfulness, further studies focus on whether the verbalized CoT accurately reflects the model's internal computational process. Emerging evidence suggests significant divergence between the reasoning traces that models generate and their underlying mechanisms.
% \textcolor{blue}{[4]}:
\citet{stechly2025beyond} demonstrates in the synthetic settings of the maze navigation problem that the connection between the CoT validity and the correctness of the final solution is weak.
Models frequently arrive at correct solutions despite generating invalid reasoning traces. Moreover, training on corrupted or semantically irrelevant traces does not damage performance. This suggests that CoT may not function as a causal mechanism for correct answer generation.
% \textcolor{blue}{[5]}:
\citet{wang2025thinking} further extracts the deception vector through representation engineering, which can control the model's deception behavior. This demonstrates that internal representations can be manipulated to induce unfaithful reasoning.

% \textcolor{blue}{[8]}(alignment):
In the context of model alignment, \citet{chan2025can} investigates whether reasoning traces may provide early signals of final response alignment before the final output. While the CoTs are unfaithful and misleading as shown in the previous paragraph, \citet{chan2025can} finds through linear probes on latent representations provide a more reliable predictive signal of alignment than the CoT texts, which indicates that the model's internal computations contain more truthful alignment signals than its verbalized reasoning.
% \textcolor{blue}{[9]}(alignment):
Similarly, \citet{yin2025refusal} identifies a \emph{refusal cliff} phenomenon in harmful prompt settings where the models are able to correctly identify harmful prompts and maintain strong refusal intentions during the thinking process, yet the intentions drop sharply right before generating the final response. This shows a misalignment between the model's internal rejection and its external output. Building on this, they propose a data selection method that targets examples with the largest refusal cliffs to realign model behavior.

\researchfinding{
The CoT in LRMs does not necessarily function as a causal mechanism for generating correct answers. Internal representations may provide more reliable signals of model intent than the verbalized reasoning.
}


\paragraph{Can We Mitigate Reward Hacking by Monitoring Chain of Thought?}

As RL increasingly incentivizes reasoning capabilities in models, reward hacking remains a fundamental problem. This naturally raises the question: can the detailed CoT produced by LRMs be effectively monitored to mitigate such hacking?
The feasibility of using CoT monitoring to mitigate reward hacking remains an open question, with studies presenting contrasting findings.
% \textcolor{blue}{[2]}:
On one hand, \citet{baker2025monitoring} shows that in agentic coding environments, CoTs can often reveal intentions of reward hacking, and such reasoning traces can be effectively detected by weaker models. Incorporating this form of supervision into the RL objective proves beneficial in low optimization settings. However, the study also cautions that excessive optimization may incentivize models to obfuscate their reasoning, thereby fostering misaligned and deceptive behaviors.
% \textcolor{blue}{[1]}:
On the other hand, \citet{dont_say_what_they_think-anthropic} offers a more skeptical view, noting that CoT monitoring does not reliably detect reward hacking, as models frequently omit such intentions from their reasoning chains. As discussed in \citet{dont_say_what_they_think-anthropic}, this more negative assessment stems from a key difference in task structure: the hacking scenarios in \citet{baker2025monitoring} require extensive exploration and complex reasoning, which naturally motivates the model to verbalize its process; in contrast, the settings in \citet{dont_say_what_they_think-anthropic} may not elicit the same level of explicit planning.
% \textcolor{blue}{[7]}:
\citet{turpin2025teaching} further confirms the limitation that RL models can engage in reward hacking without revealing it in the CoT. 
To address this issue of latent misalignment, \citet{turpin2025teaching} proposes verbalization fine-tuning---a pre-RL training stage designed to enhance contextual faithfulness by encouraging models to explicitly acknowledge when their answers are influenced by external cues.

\researchfinding{
CoT monitoring offers limited reliability against reward hacking; while it can detect hacking that requires explicit reasoning, models do not often verbalize their hacking intent in other settings.
}

% 1. Reasoning Models Don’t Always Say What They Think (Anthropic)

% 2. Chain-of-Thought Reasoning In The Wild Is Not Always Faithful (Neel Nanda)

% 3. Beyond Semantics: The Unreasonable Effectiveness of Reasonless Intermediate Tokens (ASU)

% 4. When Thinking LLMs Lie: Unveiling the Strategic Deception in Representations of Reasoning Models

% 1. Safety - Chain of Thought Monitorability: A New and Fragile Opportunity for AI Safety (OpenAI)

% 2. Training - Teaching Models to Verbalize Reward Hacking in Chain-of-Thought Reasoning (Anthropic, ScaleAI)

% 3. Alignment - Can We Predict Alignment Before Models Finish Thinking? Towards Monitoring Misaligned Reasoning Models

% 4. Alignment - Reliable Weak-to-Strong Monitoring of LLM Agents (ScaleAI)

% 5. Alignment - Refusal Falls off a Cliff: How Safety Alignment Fails in Reasoning?


\subsection{On the Tendency of CoT Reasoning to Overthink}
\label{ssec:overthink}
While long-thinking CoT reasoning helps solve complex tasks by generating additional thinking tokens, it shows a tendency to produce verbose and redundant reasoning processes, known as ``overthinking''~\citep{chen2024not, sui2025stop}. In this section, we discuss the specific patterns of overthinking and explore its possible causes and underlying mechanisms.

\paragraph{Thinking More Does Not Necessarily Lead to Better Reasoning.}
LRMs generally exhibit a test-time scaling law where performance improves with increased computational allocation, often realized through longer reasoning chains. However, a growing body of research demonstrates that this relationship is not monotonically positive;  showing instead that overly extending reasoning length can lead to performance degradation, a phenomenon widely referred to as overthinking.
Empirical studies consistently reveal a characteristic \textbf{inverse U-shaped pattern}: accuracy typically increases with reasoning length up to an optimal point, beyond which it plateaus or declines. \citet{marjanovic2025deepseek,su2025between,ghosal2025does} 
% \textcolor{blue}{DeepSeek-R1 Thoughtology}, \textcolor{blue}{Between Underthinking and Overthinking} and \textcolor{blue}{Does Thinking More Always Help?} 
chart this trajectory, showing performance peaks at a moderate thought length before considerably decreasing for excessively long generations. 
Besides, 
% \textcolor{blue}{Don't Overthink It} and \textcolor{blue}{Between Underthinking and Overthinking} 
\citet{hassid2025don, su2025between} observe that incorrect answers frequently have longer average reasoning lengths than correct ones. 
Moreover, as noted in \citet{yang2025towards}, the optimal length varies across different tasks. 

A critical insight from this body of work is that models frequently \textbf{misalign reasoning effort with problem difficulty}. 
% \textcolor{blue}{Do NOT Think That Much for 2+3=?} and \textcolor{blue}{Between Underthinking and Overthinking} 
\citet{chen2024not, su2025between} find that LRMs often generate disproportionately long solutions even for trivial problems like ``What is the answer of 2 plus 3'', yet later reasoning steps contribute marginally to accuracy. Conversely, these models may also ``underthink'' complex problems, failing to allocate sufficient reasoning depth when it is most needed. This miscalibration suggests that models struggle to assess the requisite computational effort accurately. 

Furthermore, specific task constructions in \citet{gema2025inverse} show that scaling can actively harm performance in domains like simple counting with distractors, regression tasks with spurious features or deduction tasks with constraint tracking, indicating that extended reasoning may reinforce faulty heuristics or cause models to lose focus. 
\researchfinding{
The length-performance curve for LRMs is often inverted U-shaped at the instance level, and current models are poorly calibrated in how they allocate reasoning effort---tending to overthink easy cases, underthink hard ones.
}
    
% paragraph: overthinking pattern
% 可以参考：   
% * 梳理了[Thoughts are all over the place: On the underthinking of o1-like llms.]，[Do not think that much for 2+ 3=? on the overthinking of o1-like llms]
% * `一直在不同方法之间switch，而每个方法自己可能under explore` incorrect responses often involve longer reasoning traces marked by frequent switches between different lines of thought where the model prematurely abandons promising directions—a tendency coined by [Thoughts are all over the place: On the underthinking of o1-like llms.] as under-thinking
% * `redundant check, excessive verification` On the other hand, over-thinking occurs when the model inefficiently expends resources by engaging in excessive verification or redundant checks after arriving at a final answer, contributing minimally to accuracy improvements [Do not think that much for 2+ 3=? on the overthinking of o1-like llms].
% 参考以上写法把各种不同的overthinking pattern分类连贯地串起来


% ### Do NOT Think That Much for 2+3=? On the Overthinking of o1-Like LLMs
%  * reasoning models tend to generate more solution rounds for easier math problems;  
% * for simple problems, later solutions marginally contribute to improvements in accuracy

% ### The Danger of Overthinking: Examining the Reasoning-Action Dilemma in Agentic Tasks
%  * *reasoning-action dilemma*: models must choose between engaging directly with their environment or relying on internal reasoning about potential actions and their hypothetical consequences
%  * reasoning models favor extended internal reasoning chains over environmental interaction
%  * recurring patterns: 
%    * *analysis paralysis*: the model spends excessive time planning future steps while making minimal environmental progress
%    * *rogue actions*: facing errors, the agent attempts to execute multiple actions simultaneously, breaking the environment’s sequential constraints
%    * *premature disengagement*: the agent terminates based on internal predictions rather than environmental feedback
%  *  higher overthinking scores correlate with decreased performance

% ### Thoughts are all over the place: On the underthinking of o1-like llms
% * o1-like LLMs frequently switch between different reasoning thoughts without sufficiently exploring promising paths to reach a correct solution
%   * difficulty: more frequently on harder problems
%   * pattern: lead to frequent switching between different thoughts without reaching a conclusion in each
%   * lead to performance decrease: correlates with incorrect responses due to insufficient exploration of reasoning paths (o1 consume more tokens in incorrect response than in correct ones due to much more frequent thought-switching behaviors)

% ### Let LLMs Break Free from Overthinking via Self-Braking Tuning
%    * first generate the first solution at the beginning of its reasoning process; then develop evolution solutions: primarily reflect, refine, supplement, or summarize the foundational solution, and may propose new approaches
%    * While evolution solutions grant the model self-correction and improvement capabilities, it is also where overthinking most frequently occurs


% ### Missing Premise exacerbates Overthinking: Are Reasoning Models losing Critical Thinking Skill?
% 1. patterns:
% * a specific overthinking scenario - facing ill-posed questions with missing premises (MiP), reasoning models easily engage in overthinking, spend much more tokens than the same well-defined questions; lack genuine critical thinking capabilities
% * comparison with non-reasoning backbones: LLMs not specifically trained for reasoning exhibit much better performance on the MiP scenario
% * specific patterns:  trapped in a self-doubt loop, repeatedly revisiting the question, and guessing the user intentions; 
% * Reasoning models often can notice the existence of MiP or identify it at an early stage, but they hesitate to commit to this judgment and keep outputting ineffective thinking.

% ### When Can Large Reasoning Models Save Thinking? Mechanistic Analysis of Behavioral Divergence in Reasoning
% [感觉这篇文章不太靠谱，不要写太多篇幅,就提一下模型在prompted-to-answer-directly的时候也可能re-engage-in-thinking]
% * Even when explicitly prompted to answer the question directly, the model may exhibit 3 different thinking modes: 
%    1) no-thinking: bypass further thinking as we asked to, and directly generates the answer
%    2) explicit thinking: re-engages in a thinking process and regenerate the </think> tag
%    3) implicit thinking: re-engages in additional thinking, but does not output the </think> tag
% * the three modes diverge in attention and activation patterns
% ### Thought Manipulation: External Thought Can Be Efficient for Large Reasoning Models
% 1. patterns
% * 即便在thinking tokens之间给了一段reasoning（from smaller models），但模型仍然可能resume thinking （also observed in `When Can Large Reasoning Models Save Thinking? Mechanistic Analysis of Behavioral Divergence in Reasoning`）；这个行为主要在RL-based models，在distillation-based model上，没有这样的现象
% ### Large Reasoning Models are not thinking straight: on the unreliability of thinking trajectories
% 1. patterns
%    * even when provided with ground-truth answer in the middle of reasoning, the model often generate excessive additional tokens, frequently doubting or even discarding the correct solution
%    * that reasoning models often struggle to identify valid solutions, relying on complex but fragile heuristics that do not reflect genuine reasoning

   
\paragraph{What are the patterns of overthinking?}

We summarize the common patterns of overthinking. We begin with an ideal reasoning process in long-thinking LLMs, which generally consists of three stages: (1) \textbf{Hypothesis generation}, where LLMs first propose candidate or potential solution paths; (2) \textbf{Expansion}, where LLMs expand on a solution path through step-by-step reasoning; (3) \textbf{Verification}, where LLMs reflect on and check the correctness or consistency of previous steps to confirm or revise the hypothesis. A successful reasoning process iterates through these three stages until it reaches the correct answer. We categorize the patterns of overthinking according to these three stages. 
In the hypothesis generation phase, the main pattern is the generation of lengthy and diverse candidate solutions without sufficiently exploring promising paths to reach a correct solution~\citep{wang2025thoughts}. A representative phenomenon is analysis paralysis, observed in agentic tasks~\citep{cuadron2025danger}, where LLMs produce increasingly complex action sequences without execution, thereby failing to expand further meaningful reasoning. 
In the expansion phase, the primary pattern of overthinking is excessive reasoning for simple problems. \citet{chen2024not} observe that for trivial questions like ``2+3'', long-thinking models generate responses tens or even hundreds of times longer than those of conventional LLMs. However, such excessive reasoning typically yields no significant improvement in accuracy. 
In the verification phase, the primary pattern of overthinking is the delayed termination or redirection of reasoning caused by the model’s inability to verify its own results. Specifically, on one hand, long-thinking models often fail to recognize that they have already reached the correct answer and continue redundant reasoning~\citep{chen2024not,sun2025stop,zhang2025adaptthink, zhao2025let}. 

\citet{fan2025missing} studies a specific scenario is ill-posed questions with missing premises where reasoning models exhibit a pronounced tendency to engage in excessive, unproductive deliberation in such cases. They often correctly identify the missing information at an early stage but, lacking genuine critical thinking or the confidence to halt, enter a self-doubt loop. The models repeatedly revisit the question, speculate on user intentions, and generate extensive, ineffective thinking, ultimately spending far more tokens than on well-defined questions.

Moreover, the compulsion to re-engage in thinking appears to be a deeply ingrained behavior, persisting even in contexts explicitly designed to suppress it. \citet{zhu2025can} shows that when explicitly prompted to answer directly, reasoning models may still bypass instructions and re-engage in thinking modes. Similarly, even when provided with ground-truth answers or a complete reasoning chain generated by other models, reasoning models often resume their own thinking, doubting or discarding the correct solution or the reasoning chain from others and generating excessive additional tokens~\citep{liu2025thought, cuesta2025large}.

\paragraph{What are the mechanisms of overthinking?}
We organize the findings along two principal lines of inquiry: (1) representational manifolds and steering, which investigates the latent space structure of reasoning and how to navigate it to suppress overthinking; and (2) internal conflict and self-verification, which examines the decision-making dynamics that produce unproductive reasoning cycles.

A line of work attributes overthinking to specific representational patterns inside the model. \citet{huang2025mitigating} identifies a distinct activation manifold associated with overthinking by contrasting activations from concise and verbose reasoning traces. Projecting the intervention onto this manifold dramatically improves efficacy. Besides, \citet{baek2025towards} similarly demonstrates that the ``amount'' of thinking can be modulated through activation steering. Furthermore, \citet{chen2025seal} provides a finer-grained taxonomy, identifying that execution, reflection and transition thoughts occupy distinct regions in the latent space. Steering the model's activations towards more execution-type reasoning effectively reduces unnecessary deliberation. Collectively, these works establish that overthinking is rooted in a model's navigable internal representations.
\researchfinding{
Overthinking corresponds to specific, steerable patterns in the model's activations.
}

Another body of research explains overthinking through the lens of internal decision-making conflicts and verification failures. \citet{dang2025internal} hypothesizes that upon encountering a problem, the model first forms an intuitive ``first impression''; overthinking is triggered when this initial bias conflicts with the outcome of its subsequent deliberate reasoning. They conduct intervention experiments where removing the original question after the first answer to eliminate the internal bias reduces reasoning length without harming performance, and fine-tuning that alters the model's initial bias correspondingly changes its propensity to reflect. 
Furthermore, \citet{zhang2025reasoningmodelsknowtheyre} shows that models encode the correctness of their intermediate answers in hidden states, and this information can be probed to predict answer correctness early. The inability to robustly utilize this self-verification signal is a key component of the verification-phase failures described earlier. 



% \textbf{Excessive Reasoning}
% [Overthink on simple questions]

% 1. Do NOT Think That Much for 2+3=? On the Overthinking of o1-Like LLMs

% \textbf{Redundant Reasoning Paths}
% [Continues reasoning despite having already found the correct answer]


% 1. Do NOT Think That Much for 2+3=? On the Overthinking of o1-Like LLMs

% \textbf{Analysis Paralysis}
% [generate increasingly complex action sequences but struggle to execute them systematically]

% 1. The Danger of Overthinking: Examining the Reasoning-Action Dilemma in Agentic Tasks

% \textbf{Rogue Actions}
% [generate elaborate, interdependent reasoning steps which may conflict with each other]

% 1. The Danger of Overthinking: Examining the Reasoning-Action Dilemma in Agentic Tasks



% \paragraph{What are the causes of overthinking?}

% 表面原因：self-verification or self-awareness? 
% 不知道哪条路径合理？
% 不知道自己正确与否？

% 本质原因：
% 训练：当今训练方式的side effects，只鼓励对错与否，可能会导致long-thinking（如果加上length penalty，确实思考长度能下降等，找一堆现有的工作）
% 模型：auto-regressive的模型架构就决定了模型在long-thinking的时候，受到前面token的影响，陷入错误的路径，或者有repeat的输出; 模型的long-context的能力仍然是有待提升的，模型的实际context处理长度没那么长，所以导致了其推理过程中不可避免的出现一些冗余等等。

% \textbf{Side Effects of Training Paradigms}

% 1. Stop Overthinking: A Survey on
% Efficient Reasoning for Large Language Models

% % so many papers develop new tricks on mitigating this

% \textbf{Long Context Understanding is hard}

% 1. longbench 2

% 2. LongReason: A Synthetic Long-Context Reasoning Benchmark via Context Expansion

% 3. processbench


% \textbf{Others}

% 1. Rethinking External Slow-Thinking: From Snowball Errors to Probability of Correct Reasoning

% 2. Complexity Control Facilitates Reasoning-Based
% Compositional Generalization in Transformers


% 3. ECM: A Unified Electronic Circuit Model for
% Explaining the Emergence of In-Context Learning and
% Chain-of-Thought in Large Language Model

% 4. Towards Reasoning Era: A Survey of
% Long Chain-of-Thought for Reasoning Large
% Language Models

% Bibliography entries for the entire Anthology, followed by custom entries
%\bibliography{anthology,custom}
% Custom bibliography entries only


